FunBench: Benchmarking Fundus Reading Skills of MLLMs

Multimodal Large Language Models (MLLMs) have shown significant potential in medical image analysis. However, their capabilities in interpreting fundus images, a critical skill for ophthalmology, remain under-evaluated. Existing benchmarks lack fine-grained task divisions and fail to provide modular analysis of its two key modules, i.e., large language model (LLM) and vision encoder (VE). This paper introduces FunBench, a novel visual question answering (VQA) benchmark designed to comprehensively evaluate MLLMs' fundus reading skills. FunBench features a hierarchical task organization across four levels (modality perception, anatomy perception, lesion analysis, and disease diagnosis). It also offers three targeted evaluation modes: linear-probe based VE evaluation, knowledge-prompted LLM evaluation, and holistic evaluation. Experiments on nine open-source MLLMs plus GPT-4o reveal significant deficiencies in fundus reading skills, particularly in basic tasks such as laterality recognition. The results highlight the limitations of current MLLMs and emphasize the need for domain-specific training and improved LLMs and VEs.

==> tables/benchmark.tex <==
\begin{table*}[tb!]
    \caption{\textbf{Comparison of existing benchmarks in ophthalmology}.}
    \label{tab:benchmark}
    \renewcommand{\arraystretch}{1.1}
    \centerline{
        \scalebox{0.6}{ 
            \begin{tabular}{@{}l rrrrrccccc@{}}
               \toprule
                \multirow{2}{*}{\textbf{Benchmark}} && \multirow{2}{*}{\textbf{\#Question categories}} & \multirow{2}{*}{\textbf{\#Images}} & \multirow{2}{*}{\textbf{\#Question}} & \multirow{2}{*}{\textbf{Available}}  && \multicolumn{4}{c}{\textbf{Tasks}}  \\
                \cline{8-11}
                &&&&&&& \textbf{L1: Modality recognition} & \textbf{L2: Anatomical recognition} & \textbf{L3: Lesion analysis} & \textbf{L4: Disease recognition} \\
                \midrule
                %\cline{1-5} \cline{7-10}
                
                OmniMedVQA \cite{hu2024omnimedvqa} && 5 & 13,899 & 15,461 & \CheckmarkBold && \CheckmarkBold & \CheckmarkBold & \textcolor{red}{\XSolidBrush} & \CheckmarkBold  \\
                LMOD \cite{qin2024lmod} && 2 & 21,933 & 38,662 & \textcolor{red}{\XSolidBrush} && \textcolor{red}{\XSolidBrush} & \CheckmarkBold & \textcolor{red}{\XSolidBrush} & \CheckmarkBold \\
                MOBench (proposed) && 18 & 182,217 & 1,412,386 &  \CheckmarkBold && \CheckmarkBold & \CheckmarkBold & \CheckmarkBold & \CheckmarkBold \\
                 
              \bottomrule
            \end{tabular}
        }
    }
    % \vspace{-0.3cm}
\end{table*}

==> tables/tasks.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[tb!]
\caption{\textbf{The categorization of tasks and corresponding examples}.}
\label{tab:tasks}
\centerline{
\scalebox{0.8}
{
\begin{tabular}{llllll}
\toprule
& & & question & options & ground truth  \\
\hline
\multirow{2}{*}{L1: Modality recognition}   & coarse-grained & & & & \\
\cline{2-6}
                                            & fine-grained  & & & & \\
\hline
\multirow{2}{*}{L2: Anatomical recognition} & relative position of optic disc and fovea & & & &\\
\cline{2-6}
                                            & laterality & & & & \\
\hline
\multirow{9}{*}{L3: Lesion analysis}        & \multirow{2}{*}{lesion type} & multiple label & & &  \\
                                            & & binary & & \\
\cline{2-6}
                                            & \multirow{2}{*}{lesion location} & multiple label & & & \\
                                            & & binary & &   \\
\cline{2-6}
                                            & \multirow{2}{*}{lesion relative location} & multiple label & & & \\
                                            & & binary & &  \\
\cline{2-6}
                                            & lesion area & & & & \\
\cline{2-6}
                                            & lesion relative area & & & & \\
\cline{2-6}
                                            & lesion count & & & & \\
\hline
\multirow{5}{*}{L4: Disease recognition}    & coarse-grained & & & & \\
\cline{2-6}
                                            & \multirow{2}{*}{fine-grained} & multiple label & & & \\
                                            & & binary & &   \\
\cline{2-6}
                                            & DR grading & & & & \\
\cline{2-6}
                                            & AMD grading & & & & \\
\bottomrule
\end{tabular}}}
\end{table*}
